Mine Tunnel Exploration using Multiple Quadrupedal Robots

Robotic exploration of underground environments is a particularly challenging problem due to communication, endurance, and traversability constraints which necessitate high degrees of autonomy and agility. These challenges are further exacerbated by the need to minimize human intervention for practical applications. While legged robots have the ability to traverse extremely challenging terrain, they also engender new challenges for planning, estimation, and control. In this work, we describe a fully autonomous system for multi-robot mine exploration and mapping using legged quadrupeds, as well as a distributed database mesh networking system for reporting data. In addition, we show results from the DARPA Subterranean Challenge (SubT) Tunnel Circuit demonstrating localization of artifacts after traversals of hundreds of meters. These experiments describe fully autonomous exploration of an unknown Global Navigation Satellite System (GNSS)-denied environment undertaken by legged robots.

==> Makefile <==
# @fclad
# Simple makefile to compile paper with latexmk. Change DIR_OUTPUT for
# a tmpfs path, you really don't want to use your write cycles of your
# SSD compiling a paper

NAME = main
LATEX = latexmk -pdf -bibtex -pvc -jobname=$(NAME)
DIR_OUTPUT = /tmp/Volatile

## Sources
SRC = $(NAME).tex

.PHONY	: all clean \
          essay

all 	: essay

essay 	:
	$(LATEX) $(SRC) > /dev/null

# @fclad
# A better clean is rm -rf / but that may have unintended consequences
clean	:
	@-rm -f $(DIR_OUTPUT)/$(NAME)*


==> figs/comm_stack/exchange.tex <==
\begin{tikzpicture}[font=\sffamily,thick,
  commentl/.style={text width=2.5cm, align=right},
  commentr/.style={commentl, align=left},]
  \scriptsize

  \node[] (init) {Client};
  \node[right=2cm of init] (recv) {Server};

  \draw[->] ([yshift=-0.5cm]init.south) coordinate (reqhash1o) --
    ([yshift=-.5cm]reqhash1o-|recv) coordinate (reqhash1e)
    node[pos=.55, above, sloped] {REQ\_HASH\_LIST};

  \draw[->] ([yshift=-.1cm]reqhash1e) coordinate (hashlist1o) --
    ([yshift=-.5cm]hashlist1o-|init) coordinate (hashlist1e)
    node[pos=.55, above, sloped] {HASH\_LIST};

  \draw[->] ([yshift=-.1cm]hashlist1e) coordinate (gethash1o) --
    ([yshift=-.5cm]gethash1o-|recv) coordinate (gethash1e)
    node[pos=.55, above, sloped] {REQ\_HASH\_0};

  \draw[->] ([yshift=-.1cm]gethash1e) coordinate (getdata1o) --
    ([yshift=-.5cm]getdata1o-|init) coordinate (getdata1e)
    node[pos=.55, above, sloped] {DATA\_0};

  \draw[->] ([yshift=-.1cm]getdata1e) coordinate (gethashn1o) --
    ([yshift=-0.5cm]getdata1e-|recv) coordinate (gethashn1e)
    node[pos=.55, above, sloped] {REQ\_HASH\_N};

  \draw[->] ([yshift=-.1cm]gethashn1e) coordinate (getdatan1o) --
    ([yshift=-.5cm]getdatan1o-|init) coordinate (getdatan1e)
    node[pos=.55, above, sloped] {DATA\_N};

  % \draw[->] (hashlist1e-|recv) coordinate (fin2o) --
  %   ([yshift=-.7cm]fin2o-|init) coordinate (fin2e) node[pos=.3, above,
  %   sloped] {FIN};

  % \draw[->] ([yshift=-.3cm]fin2e) coordinate (ack2o) --
  % ([yshift=-.7cm]ack2o-|recv) coordinate (ack2e) node[pos=.3, above,
  % sloped] {ACK};

  \draw[thick, shorten >=-.2cm] (init) -- (init|-getdatan1e);
  \draw[thick, shorten >=-.2cm] (recv) -- (recv|-getdatan1e);

  \draw[dotted] (recv.285)--([yshift=2mm]recv.285|-reqhash1e)
  coordinate[pos=.5] (aux1);

  \draw[dotted] (init.255)--([yshift=2mm]init.255|-reqhash1o);

  % \draw[dotted] ([yshift=1mm]init.255|-fin2e)
  % --([yshift=-5mm]init.255|-ack2e) coordinate (aux2);

  % \node[commentr, right =2mm of ack2e] {\textbf{CLOSED}};
  % \node[commentr, right =2mm of fin2o] {\textbf{LAST ACK}};

  % \node[below left = 0mm and 2mm of init.south,
  % commentl]{\textbf{ESTABLISHED}\\[-1.5mm]{\itshape connection}};
  \node[left = 2mm of reqhash1o.west, commentl]
  {{\itshape Request hash list}};
  \node[left = 2mm of hashlist1e.west, commentl]
  {\textbf{Compare remote and local hashes}\\
  {\itshape Request first different hash with higher priority}};
  \node[left = 2mm of getdata1e.west, commentl]
  {\textbf{Commit data into DB}\\
  {\itshape Request next different hash}};
  \node[left = 2mm of getdatan1e.west, commentl]
  {\textbf{Commit data into DB}};
  % \node[below left = -1mm and 2mm of fin2e.west,
  % commentl]{\textbf{TIME\_WAIT}};
  % \node[below left = -1mm and 2mm of aux2-|init,
  % commentl]{\textbf{CLOSED}};

  % \node[right = 2mm of recv|-aux1,
  % commentr]{\textbf{ESTABLISHED}\\[-1.5mm]{\itshape connection}};
  \node[right = 2mm of reqhash1e.west, commentr]
  {\textbf{Get hashes DB}\\
  {\itshape Send hash list}};
  \node[right = 2mm of getdata1o.west, commentr]
  {\textbf{Fetch from DB}\\
  {\itshape Send requested data}};
  \node[right = 2mm of getdatan1o.west, commentr]
  {\textbf{Fetch from DB}\\
  {\itshape Send requested data}};

\end{tikzpicture}

